Overlooked factors in concept-based explanations: Dataset choice, concept learnability, and human capability

Concept-based interpretability methods aim to explain deep neural network model predictions using a predefined set of semantic concepts. These methods evaluate a trained model on a new, "probe" dataset and correlate model predictions with the visual concepts labeled in that dataset. Despite their popularity, they suffer from limitations that are not well-understood and articulated by the literature. In this work, we analyze three commonly overlooked factors in concept-based explanations. First, the choice of the probe dataset has a profound impact on the generated explanations. Our analysis reveals that different probe datasets may lead to very different explanations, and suggests that the explanations are not generalizable outside the probe dataset. Second, we find that concepts in the probe dataset are often less salient and harder to learn than the classes they claim to explain, calling into question the correctness of the explanations. We argue that only visually salient concepts should be used in concept-based explanations. Finally, while existing methods use hundreds or even thousands of concepts, our human studies reveal a much stricter upper bound of 32 concepts or less, beyond which the explanations are much less practically useful. We make suggestions for future development and analysis of concept-based interpretability methods. Code for our analysis and user interface can be found at \url{https://github.com/princetonvisualai/OverlookedFactors}

==> sections/old_conclusion.tex <==
% Summary
In this work we examine implicit assumptions made in concept-based interpretability methods. We consider 3 aspects of these assumptions: the choice of the probe dataset, the concepts used for the explanations, and use to humans. We find that the choice of dataset profoundly affects the explanation output, implying that these explanations can only be used for images from the probe dataset distribution. We also find that a significant fraction of the concepts used within explanations are harder to learn for a model than the concepts they claim to explain. Finally, from a practical standpoint, we find that humans struggle to identify concepts within images, and the majority of them prefer that explanations have no more than 32 concepts.

% Limitations and potential negative impact
A limitation of our work is that we are only able to test each of the methods on a single setting, for example, we only test NetDissect~\cite{bau2017netdissect}, TCAV~\cite{kim2018tcav} and IBD~\cite{zhou2018ibd} on a scene classifier trained on Places365~\cite{zhou2017places}. This is due to a lack of other available probe datasets. %\vikram{Are there other limitations? I think this is the main one} \sunnie{Agreed!}
We stress that these tests are not sufficient to validate human intuitions regarding the probe dataset or concepts to be used, however, they are necessary. A potential negative impact of our work would be for researchers to claim that the probe dataset or the concepts used are `correct' based on the results of our analysis. We also emphasize that our findings are not to suggest that the concept-based explanations should not be used. %Rather, we believe that these findings provide practitioners with additional considerations to keep in mind when designing and using concept-based explanations. We hope that our work provides 
We hope that our work provides researchers with additional tools to evaluate concept-based interpretability methods, thereby ensuring that these methods are more applicable. 

%and  suggestions assists practitioners with  Moreover, we offer concrete suggestions for the community going forward

%\sunnie{General comments about Sections 6 and 7: (1) I think they can be shorter and maybe even combined into one section? (2) Since there are separate checklist items for ``limitations" and ``potential negative societal impacts," should we explicitly use these terms? (That said I'm not sure what we'd write for potential negative societal impacts...) (3) Should we end the paper on a more positive note and/or in a way that highlights our contributions?}\vikram{agree about the third, we are using the terms right now? Or do you mean like within a smallsec}

==> sections/old_human_exp_beforemay16.tex <==
Within the last two sections, we analysed the probing dataset used, as well as the actual concepts used to generate explanations. In this last section, we propose tests to understand the usefulness of these explanations to humans. In particular, we focus on the complexity of these explanations. 

In the past, concept-based explanations have tried to use as many attributes as are available within the probing dataset: NetDissect~\cite{bau2017netdissect} and Net2Vec~\cite{fong2018net2vec} use all 1197 concepts labelled within the Broden~\cite{bau2017netdissect} dataset; IBD~\cite{zhou2018ibd} uses all object and part labels within Broden with at least 10 examples (660 concepts), Concept Bottleneck~\cite{koh2020conceptbottleneck} uses all labels with over XX examples from CUB~\cite{WahCUB_200_2011} (112 concepts). However, asking humans to reason about these many concepts seems daunting. We propose tests to understand how many concepts humans can reason about, and ask if humans are willing to trade-off completeness of the explanation (i.e, how much of the model is explained using a specific method) for a simpler explanation.  

\subsection{Study design}
 We ask the participants to perform three tasks to understand how well humans can digest concept-based explanations and learn their preferences regarding explanation simplicity vs explanation completeness. 

\smallsec{Task 1: Simulating the explanations} Similar to prior works like \citet{poursabzi2021manipulating}, we measure how well humans are able to digest explanations by asking them to simulate a model's behaviour given access to the explanation. Since the explanations we consider are concept-based, we ask participants to identify the presence / absence of concepts used within the model given a new input. We generate explanation scores based on the concepts selected. Fig~\ref{fig:ui_simulation} shows an example of the UI designed. This type of explanation is similar to the ones generated by generated by IBD, Baseline and Concept Bottleneck. 

\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{figures/ui_checkbox_220424.png}
    \caption{\textbf{UI design - Explanation simulation}. We show a new image and ask participants to simulate the explanation by choosing concepts that are present. \vikram{Sunnie, can you update this with the current UI image?}}
    \label{fig:ui_simulation}
\end{figure}

In order to ensure that our subjects only consider the explanation complexity (and not the model complexity), we generate explanations when using just 4 classes, rather than the 365 present in Places365, asking participants to choose between these 4. All explanations are generated using the Baseline method, however, we note that the method used to generate the explanation does not impact the user's ability to simulate the model. 

We use 2 different sets of 4 classes from Places 365, and vary the complexity of the explanations by changing the number of concepts used by the explanation (8, 16 and 32). Since our goal is to understand how humans reason about these explanations, we only use example images where the blackbox model's output and the explanation agree. For this task, we measure the time taken by participants to complete this task, as well as their accuracy.

\smallsec{Task 2: Agreement with the concepts used within the explanation} \vikram{I'm confused about why exactly we're doing this task?}

\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{figures/ui_agreement.png}
    \caption{\textbf{UI design - Concept agreement}\vikram{Sunnie, can you update this with the current UI image?}}
    \label{fig:ui_concept}
\end{figure}


\smallsec{Task 3: Trade-off between simplicity and completeness}. Finally, we ask participants to reason about how much they value simple explanations over explanations that explain a majority of the model's prediction. We show participants sample graphs of how the fraction of the model explained can change when using explanations of differing complexities, and ask them to choose the explanation they prefer. 



==> sections/old_setup.tex <==
In this section, we provide details on the different concept-based methods we investigate, along with a simple baseline explanation method. We also provide other details regarding our experiments that remain constant across the different sections. 

\subsection{Explanation methods} We choose 5 different popular concept-based explanation methods: \textbf{NetDissect}~\cite{bau2017netdissect}, \textbf{TCAV}~\cite{kim2018tcav}, \textbf{Net2Vec}~\cite{fong2018net2vec}, \textbf{IBD}~\cite{zhou2018ibd} and \textbf{ConceptBottleneck}~\cite{koh2020conceptbottleneck}. We also consider a simple baseline explanation method, that we call \textbf{Baseline}.

\smallsec{NetDissect~\cite{bau2017netdissect}} Bau et al. identify neurons within the network that are highly activated by certain concepts. By thresholding activation maps at the 99.5\% percentile, they measure the IOU with a ground truth segmentation of the concept. They consider a neuron to be highly activated by an concept if this IOU$>0.04$. 

\smallsec{Net2Vec~\cite{fong2018net2vec}} Fong et al. learn concept vectors that are used to linearly combine activations from individual neurons to perform a given task (e.g. concept segmentation or classification). They study how concept vectors learned using all neurons in a layer compare to using smaller subsets of neurons as well as using just a single neuron, as done in NetDissect~\cite{bau2017netdissect}.

\smallsec{TCAV~\cite{kim2018tcav}} Kim et al. learn directions within the feature space that correspond to different concepts. With this, they are able to compute the relative importance of the model's prediction with respect to an concept. 

\smallsec{IBD~\cite{zhou2018ibd}} Zhou et al. greedily learn a basis of concept vectors as well as a residual vector such that any model prediction can be decomposed into a linear combination of the basis and residual vectors (i.e. a linear model). Then, for a specific prediction, they compute how much each concept contributes to the prediction and shows attribution heatmaps (i.e. CAM~\cite{zhou2016cam} or GradCAM~\cite{selvaraju2017gradcam}) for each contributing concept.

%\vikram{Maybe not concept bottleneck?}
\smallsec{Concept Bottleneck~\cite{koh2020conceptbottleneck}} Unlike the other interpretability methods we consider, Concept Bottleneck is an \emph{interpretable-by-design} method, meaning that the model is trained to be interpretable.
Here, Koh et al. construct a model that first learns to predict a set of concepts, and then learns a linear layer with the concepts to predict the final class.
Concept Bottleneck models allow for concept scores to be fractional, since these scores are continuous values output by the model.%\ruth{skipped on pass}  

\smallsec{Baseline} For the baseline, we learn a logistic regression model that predicts the model's output given access to ground truth concepts within the image. This is similar to the linear model in IBD as well as Concept Bottleneck. We include this model as a simple example that learns correlations between concepts and classes. This allows us to compare the results of our sanity checks between methods that heavily depend on internal scores of the model with  one that does not. 
%We include this baseline as a sanity check.\ruth{maybe different term and motivate a bit more why we're using this?} 


\subsection{Models}
We generate explanations for two different models: a Places365~\cite{zhou2017places} trained ResNet18~\cite{he2016resnet} model and a Concept Bottleneck model~\cite{koh2020conceptbottleneck} trained on the CUB dataset~\cite{WahCUB_200_2011}.
We choose these two models since all the interpretability methods we study have been evaluated on one of these two models. 

\subsection{Probing datasets}
Concept-based explanations require access to a set of images labelled with concepts, that are typically not in the training dataset.
Similar to prior works, when generating explanations for the Places365 trained ResNet18 model, we use the Broden dataset~\cite{bau2017netdissect}.
This dataset is comprised of multiple datasets (Pascal-Context~\cite{mottaghi2014role}, Pascal-Part~\cite{chen2014detect}, ADE20k~\cite{zhou2017ade20k,zhou2019ade20k_ijcv}, OpenSurfaces~\cite{bell2014intrinsic} and Describable Textures Dataset~\cite{cimpoi2014describing}) and includes labels for a total of 1197 distinct concepts, which each belong to one of the following cateogries: color, texture, material, object, part, and scene.
The concept annotations provide image-level labels (for texture and scene concepts) and pixel-level segmentation masks (for all other concepts).
%These concepts belong to one of 5 categories: color, texture, material, object, part, and scene.
For this work, since we explain scene classification, we use the ADE20k and Pascal subsets of the dataset, labelled with objects and parts. 
When generating explanations for models trained on the CUB dataset, we use the CUB test split, along with the labelled concepts provided in CUB.
This setting is unique in that the training and probing datasets are from similar distributions, both labelled with a total of 200 concepts.
We use the subset of 112 concepts used in Concept Bottleneck. 


==> sections/suppmat.tex <==
\appendix

\section*{Overlooked factors in concept-based explanations: Dataset choice, concept salience, and human capability (Paper 3678) - Supplementary material}

In this supplementary document, we provide additional
details on some sections of the main paper.

\begin{itemize}[leftmargin=0pt, itemsep=1pt, topsep=1pt]
\item[] \textbf{Section \ref{sec:supp-humanstudy}:} We supplement Section 5 of the main paper and provide more information about our human studies.
\item[] \textbf{Section \ref{sec:supp-ui}:} We supplement Section 5 of the main paper and show snapshots of our full user interface.
\end{itemize}

\section{Human study details}
\label{sec:supp-humanstudy}

In Section 5 of the main paper, we discuss the human studies we ran to understand how well humans are able to reason about concept-based explanations as the number of concepts used within the explanation increases. 
% Our key finding is that participants struggle to identify relevant concepts as the number of concepts increases and the majority of participants prefer that the number of concepts be limited to 32.
In this section, we provide additional details.

To recap, we compare four types of explanations: (1) concept-based explanations that use 8 concepts, (2) concept-based explanations that use 16 concepts, (3) concept-based explanations that use 32 concepts, and (4) example-based explanations that consist of 10 example images for which the model predicts a certain class.
(4) is a baseline that doesn't use concepts.

For a fair comparison, all four types of explanations are evaluated on the same inputs.
We generate five sets of input where each set consists of 5 images from one scene group (commercial buildings, shops, markets, cities, and towns) and 5 images from another scene group (home or hotel). 
Recall that these are images where the model output match the explanation output (i.e., the class with the highest explanation score calculated based on ground-truth concept labels).
Hence, if the participants correctly identify all concepts that appear in a given image, they are guaranteed to get the highest explanation score for the model output class.
% since our goal is to understand how humans reason with concept-based explanations with varying complexities.

To reduce the variance with respect to the input, we had 5 participants for each set of input and explanation type.
For 32 concepts explanations, each participant saw 5 images from only one of the two scene groups because the study got too long and overwhelming with the full set of 10 images.
For all other explanations, each participant saw the full set of 10 images.
In total, we had 125 participants: 50 participants for the study with 32 concepts explanations and 25 participants for the other three studies.
Each participant sees only one type of explanation as we conduct a between-group study.

More specifically, we recruited participants through Amazon Mechanical Turk who are US-based, have done over 1000 Human Intelligence Tasks, and have prior approval rate of at least 98\%. 
The demographic distribution was: man 59\%, woman 41\%; no race/ethnicity reported 82\%, White 17\%, Black/African American 1\%, Asian 1\%.
The self-reported machine learning experience was 2.5 $\pm$ 1.0, between ``2: have heard about...'' and ``3: know the basics...'' 
We did not collect any personally identifiable information. 
Participants were compensated based on the state-level minimum wage of \$12/hr. In total, $\sim$\$800 was spent on running human studies.


\section{User interface snapshots}
\label{sec:supp-ui}

In Section 5.1 of the main paper, we outlined our human study design.\footnote{We note that much of our study design and UI is based on the recent work by Kim et al.~\cite{kim2021hive} who propose a human evaluation framework called HIVE for evaluating visual interpretability methods.}
Here we provide snapshots of our study UIs in the following order.

\textbf{Study introduction.} For each participant, we introduce the study, present a consent form, and receive informed consent for participation in the study. The consent form was approved by our institution's Institutional Review Board and acknowledges that participation is voluntary, refusal to participate will involve no penalty or loss of benefits, etc.
See~\cref{fig:ui_study_intro}.

 
\textbf{Demographics and background.} Following HIVE~\cite{kim2021hive}, we request optional demographic data regarding gender identity, race and ethnicity, as well as the participant's experience with machine learning. We collect this information to help future researchers calibrate our results.
See~\cref{fig:ui_demographic_background}.


\textbf{Method introduction.} We introduce concept-based explanations in simple terms. This page is not shown for the study with example-based explanations.
See~\cref{fig:ui_method_intro}.


\textbf{Task preview } We present a practice example to help participants get familiar with the task. This page is not shown for the study with example-based explanations.
See~\cref{fig:ui_task_preview}.


\textbf{Part 1: Recognize concepts and guess the model output} After the preview, participants move onto the main task where they are asked to recognize concepts in a given photo (for concept-based explanations) and predict the model output (for all explanations). We show the UI for each type of explanation we study:
\begin{itemize}%[leftmargin=0pt, itemsep=1pt, topsep=1pt]
\item 8 concept explanations (\cref{fig:ui_task_8concept})
\item 16 concepts explanations (\cref{fig:ui_task_16concept})
\item 32 concepts explanations (\cref{fig:ui_task_32concept})
\item Example-based explanations (\cref{fig:ui_task_example})
\end{itemize}


\textbf{Part 2: Choose the ideal tradeoff between simplicity and correctness.} 
Concept-based explanations can have varying levels of complexity/simplicity and correctness. Hence, we investigate how participants reason with these two properties. To do so, we show examples of concept-based explanations that use different numbers of concepts, as well as bar plots with the correctness values for certain instantiations of concept-based explanations.
We then ask participants to choose the explanation they prefer the most and provide a short written justification for their choice.
See~\cref{fig:ui_tradeoff}.


\textbf{Feedback.} At the end of the study, participants can optionally provide feedback. See~\cref{fig:ui_feedback}.


\clearpage

% \iffalse

\begin{figure*}[t!]
\centering
\includegraphics[width=0.8\linewidth]{figures_suppmat/ui_study_intro.png}
\caption{\textbf{UI - Study introduction}}
\label{fig:ui_study_intro}
\vspace{2cm}
\includegraphics[width=0.75\linewidth]{figures_suppmat/ui_demographics_background.png}
\caption{\textbf{UI - Demographics and background}}
\label{fig:ui_demographic_background}
\end{figure*}


\begin{figure*}[t!]
\centering
\includegraphics[width=\linewidth]{figures_suppmat/ui_method_intro_1.png}
\includegraphics[width=\linewidth]{figures_suppmat/ui_method_intro_2.png}
\caption{\textbf{UI - Method introduction}}
\label{fig:ui_method_intro}
\end{figure*}

\begin{figure*}[t!]
\centering
\includegraphics[width=\linewidth]{figures_suppmat/ui_task_preview.png}
\caption{\textbf{UI - Task preview}}
\label{fig:ui_task_preview}
\end{figure*}


\begin{figure*}[t!]
\centering
\includegraphics[width=\linewidth]{figures_suppmat/ui_task_8concept_1.png}
\includegraphics[width=\linewidth]{figures_suppmat/ui_task_8concept_2.png}
\caption{\textbf{UI - Part 1: Recognize concepts and guess the model output (8 concepts explanations)}}
\label{fig:ui_task_8concept}
\end{figure*}


\begin{figure*}[t!]
\centering
\includegraphics[width=\linewidth]{figures_suppmat/ui_task_16concept_1.png}
\includegraphics[width=\linewidth]{figures_suppmat/ui_task_16concept_2.png}
\caption{\textbf{UI - Part 1: Recognize concepts and guess the model output (16 concepts explanations)}}
\label{fig:ui_task_16concept}
\end{figure*}


\begin{figure*}[t!]
\centering
\includegraphics[width=\linewidth]{figures_suppmat/ui_task_32concept_1.png}

\vspace{0.5cm}

\includegraphics[width=\linewidth]{figures_suppmat/ui_task_32concept_2.png}
\includegraphics[width=\linewidth]{figures_suppmat/ui_task_32concept_3.png}
\caption{\textbf{UI - Part 1: Recognize concepts and guess the model output (32 concepts explanations)}}
\label{fig:ui_task_32concept}
\end{figure*}

\begin{figure*}[t!]
\centering
\includegraphics[width=\linewidth]{figures_suppmat/ui_task_example_1.png}
\includegraphics[width=\linewidth]{figures_suppmat/ui_task_example_2.png}
\caption{\textbf{UI - Part 1: Guess the model output (example-based explanations)}}
\label{fig:ui_task_example}
\end{figure*}


\begin{figure*}[t!]
\centering
\includegraphics[width=\linewidth]{figures_suppmat/ui_tradeoff1.png}
\includegraphics[width=0.7\linewidth]{figures_suppmat/ui_tradeoff2.png}
\includegraphics[width=\linewidth]{figures_suppmat/ui_tradeoff3.png}
\caption{\textbf{UI - Part 2: Choose the ideal tradeoff between simplicity and correctness}}
\label{fig:ui_tradeoff}
\end{figure*}


\begin{figure*}[t!]
\centering
\includegraphics[width=0.85\linewidth]{figures_suppmat/ui_feedback.png}
\caption{\textbf{UI - Feedback}}
\label{fig:ui_feedback}
\end{figure*}

% \fi
